Dialogue-Contextualized Re-ranking for Medical History-Taking

AI-driven medical history-taking is an important component in symptom checking, automated patient intake, triage, and other AI virtual care applications. As history-taking is extremely varied, machine learning models require a significant amount of data to train. To overcome this challenge, existing systems are developed using indirect data or expert knowledge. This leads to a training-inference gap as models are trained on different kinds of data than what they observe at inference time. In this work, we present a two-stage re-ranking approach that helps close the training-inference gap by re-ranking the first-stage question candidates using a dialogue-contextualized model. For this, we propose a new model, global re-ranker, which cross-encodes the dialogue with all questions simultaneously, and compare it with several existing neural baselines. We test both transformer and S4-based language model backbones. We find that relative to the expert system, the best performance is achieved by our proposed global re-ranker with a transformer backbone, resulting in a 30% higher normalized discount cumulative gain (nDCG) and a 77% higher mean average precision (mAP).

==> sections/method.old.tex <==
\section{Methods}
\label{sec:method}


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/hx-taking-reranking.drawio.png}
    \caption{Overview of the history-taking workflow. An expert system suggests candidate questions based on relevant entities extracted from the dialogue. A machine-learned deep neural network re-ranker then re-ranks the candidate questions based on the dialogue text.}
    \label{fig:flow}
    \vspace{-1em}
\end{figure}

An overview of our approach can be seen in \autoref{fig:flow}. We first use an expert system to suggest relevant history-taking questions, and then use a deep neural network contextualized by the entire \doctor-patient dialogue to re-rank expert system suggestions.



\subsection{Task description}

The goal of re-ranking is,  given the prior dialogue context $\boldsymbol{d}$ and a list of $n$ candidate history-taking questions $Q=[\boldsymbol{q}_1, \boldsymbol{q}_2, \dots, \boldsymbol{q}_n]$, to generate a new list $Q'$ which consists of (possibly reordered) questions from $Q$ such that the higher relevance questions appear earlier in the sequence. In our case, the candidate questions are generated using an in-house Expert System, and the ground truth labels $\boldsymbol{y}=[y_1,y_2,\dots,y_n], y_i\in\{0,1\}$ represent whether a \doctor~asked a given recommended question ($1$ if the question was asked, $0$ if the question was not asked). A doctor may ask multiple questions at the same time, thus multiple elements of $\boldsymbol{y}$ can have a value of $1$, see \S~\ref{sec:data} for more details on how the ground truth is produced. Finally, in all of the models studied in this work, the re-ranking is achieved by assigning scores $\boldsymbol{s}=[s_1,s_2,\dots,s_n]$ to each question in $Q$, and then constructing $Q'$ by reordering using scores in $\boldsymbol{s}$.


% Here we only consider binary relevance, in which $y_i=1$ means that the candidate question $q_i$ is selected by a physician in an actual medical dialogue whereas $y_i=0$ implies that $q_i$ is not selected. However, the actual number of relevant questions are flexible, as the physician can select multiple history-taking questions at once. The goal is to predict a list of scores $\boldsymbol{s}=[s_1,s_2,\dots,s_n]$ that approximates the ranking of the ground truth $\boldsymbol{y}$. While $\boldsymbol{y}$ only contains binary values, there is not limit in the range of $\boldsymbol{s}$. Each score $s_i$ can take any range values as long as the magnitude of the value reflects the true ranking in $\boldsymbol{y}$. 


\subsection{Global re-ranker}
\label{sec:global-re-ranker}

We propose the global re-ranker, an accurate and efficient listwise ranking method. 
%Unlike prior pointwise approaches that only consider a query and a document at a time, the groupwise/listwise approach incorporates the interactions between candidate documents, therefore achieving better ranking results \cite{chen2021co,ai2019learning}. 
In this approach (see \autoref{fig:models}(c) for a schematic), the history-taking dialogue and all candidate history-taking questions are concatenated into a single text input, using which the model then assigns the ranking scores to all questions simultaneously. The global re-ranker directly encodes all texts through the language model, thereby ensuring deep semantic interactions not only between the dialogue and the candidate questions but also between all candidate questions. 

% While directly encoding more than one candidates with a given query has been explored in duoBERT \cite{nogueira2019multi} and duoT5 \cite{pradeep2021expando}, these models only investigate pairwise scoring due to length constraints imposed by the pretrained transformer. In our approach, this challenge can be addressed by the adoption of long-range transformers, which are highly efficient in processing long textual sequences. MOVED TO RELATED WORK

% Like the cross-encoder, the global re-ranker models the interactions between the dialogue and the candidate questions by fusing them in early layers. Therefore it learns the relations between contexts and questions better than the bi-encoder architecture, which encodes them separately without interactions. However, one disadvantage of the cross-encoder is that it only scores each question in isolation and ranks them in a {\it post hoc} manner, which prevents it from learning the relations between candidate questions. In a typical ranking task, the ranking system should not only indicate which question is relevant but also which question is preferred over other questions.  As the global re-ranker ranks a list of questions in a single pass, it is more computationally efficient than the cross-encoder, which has to perform $n$ rounds of inference for a list of $n$ candidate questions. EITHER FULL REMOVAL OR WILL MOVE

% In the global re-ranker, the goal is to train a neural model $f_G$ that scores all candidate questions simultaneously given the dialogue context.

% \begin{equation}
%     s_1,s_2,\dots,s_n = f_{G}(\boldsymbol{d}, \boldsymbol{q}_1, \boldsymbol{q}_2, \dots, \boldsymbol{q}_n)
% \end{equation}

The input text to the global re-ranker is the concatenation of both the dialogue context and all the candidate questions: \texttt{[CLS]} $\boldsymbol{d}$ \texttt{[SEP]} $\boldsymbol{q}_1$ \texttt{[MASK\textsubscript{1}][SEP]} $\boldsymbol{q}_2$ \texttt{[MASK\textsubscript{2}]}\texttt{[SEP]} \dots  $\boldsymbol{q}_n$ \texttt{[MASK\textsubscript{n}][SEP]}, 
where the \texttt{[SEP]} token is used to mark the boundaries of candidate questions. The \texttt{[MASK\textsubscript{i}]} token is the pooling token for the preceding question $\boldsymbol{q}_i$. For each pooling token \texttt{[MASK\textsubscript{i}]}, the global reranker predicts a score $s_i$, which represents the relevance for $\boldsymbol{q}_i$. We also added type embeddings to every input tokens to indicate whether it belongs to the dialogue or the candidate questions. 

While self-attention itself does not assume any inherent order of the input sequence, pretrained transformer models usually encode the text sequentially due to the presence of positional embeddings. In the current task, it is expected that a language model learns the sequential relations between words within $\boldsymbol{d}$ and $\boldsymbol{q}_i$. From our ablation experiments (see \S~\ref{sec:ablations}, we found that the best performance is achieved when the model is agnostic to the order of input questions $[\boldsymbol{q}_1, \boldsymbol{q}_2, \dots, \boldsymbol{q}_n]$. In order to remove the positional bias, we reset the positional embedding when each new question starts. 
 
We selected three different neural architectures to implement the global ranker, all of which can process long textual sequences. The first two approaches are based on the Nystromformer \cite{xiong2021nystromformer}, which was originally proposed to be an efficient transformer. We experiment with Nystromformer with both Nystrom attention turned on and turned off (in which case it uses full attention). We use Nystromformer as the base of our ``full attention'' transformer because this enables us to leverage the pretrained Nystromformer checkpoints that had been trained on long texts and retain the good performance of full attention. We learned from pilot experiments that other efficient transformers such as Longformer \cite{beltagy2020longformer} failed to converge. The third neural architecture is a state-space model, S4, which has been shown to process long sequences more effectively than many transformers \cite{gu2021efficiently}.

To train the global re-ranker, we compared a variety of loss functions across point-wise, pair-wise and listwise approaches in the learning-to-rank framework \cite{liu2009learning}. The point-wise baseline was trained with binary cross-entropy. For pairwise loss functions, we tested the RankNet \cite{burges2005learning} and LambdaRank \cite{burges2006learning}. The listwise loss functions we used were ListNet \cite{cao2007learning}, ListMLE \cite{xia2008listwise}, ApproxNDCG \cite{qin2010general} and NeuralNDCG \cite{Pobrotyn2021NeuralNDCG}, the latter two of which directly optimized the Normalized Discounted Cumulative Gain (NDCG) metrics. 






\subsection{Baseline approaches} 
In addition to the global ranker, we also implement several widely adopted baseline ranking approaches. 

\paragraph{Bi-encoder.} In the bi-encoder architecture (see Figure~\ref{fig:models}(a)), the dialogue query and the candidate questions are encoded by two separate encoders $f_D$ and $f_Q$, the relevance score between the two resulting vector representations are computed with cosine similarity. The bi-encoder learns an embedding space where the dialogue representation is close to the most relevant questions while being distant from less relevant questions. The training objective is to minimize the InfoNCE loss function \cite{oord2018representation} through contrastive learning. The temperature parameter of the InfoNCE loss was set to 0.05 throughout the training \cite{gao-etal-2021-simcse}. 

\paragraph{Cross-encoder.} In the cross-encoder architecture (see Figure~\ref{fig:models}(b)) the prior dialogue is concatenated with a candidate question. The cross-encoder $f_C$ assigns a relevance score to this candidate question. We considered transformers and S4-based models. For transformers, the \texttt{[CLS]} token was treated as the contextual representation of the dialogue and the query. A classification head projected the contextual representation into a relevance score. The cross-encoder is trained with the binary cross-entropy loss. For the bi-redictional S4 re-rankers, average pooling was used to obtain the fixed-dimensional contextual representations. 

\paragraph{Autoregressive re-ranker.} We also consider autoregressive re-rankers\cite{nogueira-etal-2020-document,pradeep2021expando}. In autoregressive re-ranking, the backbone of the re-ranker is a sequence-to-sequence transformer, such as T5 \cite{raffel2020exploring} and LongT5 \cite{guo2021longt5}. The query and the document are concatenated together to form the input sequence: \texttt{Query:} $d$ \texttt{Document:} $q_i$ \texttt{Relevant:}, which is fed into the encoder. Then the transformer decoder predicts either \texttt{true} or \texttt{false} as the target word (\texttt{true} for relevant documents whereas \texttt{false} for irrelevant documents). During inference, a softmax function is applied to the logits of the \texttt{true} and the \texttt{false} tokens, and the resulting probability of the \texttt{true} token is treated as the relevance score. For autoregressive S4 re-ranker, however, the setting is the same as the cross-encoder, except that the underlying model is autoregressive rather than bi-directional. The concatenated dialogue and a candidate question were fed into the S4 re-ranker and the average pooling of the last layer is classified as either relevant or irrelevant through a classification head. \TODO{Jian, can you confirm this para, also should we explain why we didn't just do it like in T5?}

\subsection{Implementation} 
\paragraph{S4 model pretraining.} The S4 model was based on the original implementation of S4 language model\cite{gu2021efficiently}, in which the S4 layers were used as a drop-in replacement for the self-attention layers in a typical transformer. We implemented a 12-layer bidirectional S4 model as the cross-encoder or the global reranker. We set the hidden dimensions to 768 in order to match the parameter count of mainstream pretrained transformers (such as BERT-base \cite{devlin-etal-2019-bert}), and the number of state-space machines (SSM) to 128 with 64 states for each SSM. The S4 model was initialized with pretrained weights. 
Both bidirectional S4 and autoregressive S4 models were pretrained on large-scale texts. The autoregressive S4 was pretrained with the casual language modeling task on the whole English subset of Wikipedia. The second iteration of pretraining, initialized with the pretrained Wikipedia checkpoint, was on the whole Pubmed PMC Open Access Subset. The bidirectional S4 models were pretrained on the same datasets but with the mask language modeling task using the same masking settings as in BERT \cite{devlin-etal-2019-bert}. The maximum sequence length for pretraining was set to 8192 and the effective batch size was 256. All models were optimized with AdamW optimizer with a learning rate of 1e-4 and the learning rate was dynamically adjusted using the Cosine Scheduler with a warm-up step of 1000. The pretraining took place on 8$\times$RTX 3090 GPU with 24GB of memory. The training was stopped when the evaluation loss stopped to decrease ($\sim$12k steps for all models). The autoregressive and bi-direction checkpoints pre-trained on these datasets will be released together with this paper.

Transformer models were all implemented through the \texttt{Transformers} package \cite{wolf2020transformers} with default dimensions. The autoregressive model was the LongT5 model \cite{guo2021longt5} initialized by the \texttt{long-t5-tglobal-base} checkpoint. Other transformers were based on the Nystromformer \cite{xiong2021nystromformer} with initialization from the public checkpoint \texttt{uw-madison/nystromformer-4096}.

For global re-rankers, the maximum input length was set to 4096 with an effective batch size of 32. For the rest of the models, the effective batch size was 64 and the maximum length was 2048, as this length was enough to cover almost all of the data samples. Models were trained with a maximum of 5 epochs and only the model with the best validation performance was kept. 
All models were trained using the AdamW optimizer \cite{loshchilov2018decoupled} with a learning rate of 5e-5. We used a cosine scheduler with a warm-up step of 1000 to automatically adjust the learning rate during training. All ranking models were trained on a single V100 GPU with 16GB of memory. 

